Denoising Score Distillation: From Noisy Diffusion Pretraining to One-Step High-Quality Generation

Diffusion models have achieved remarkable success in generating high-resolution, realistic images across diverse natural distributions. However, their performance heavily relies on high-quality training data, making it challenging to learn meaningful distributions from corrupted samples. This limitation restricts their applicability in scientific domains where clean data is scarce or costly to obtain. In this work, we introduce denoising score distillation (DSD), a surprisingly effective and novel approach for training high-quality generative models from low-quality data. DSD first pretrains a diffusion model exclusively on noisy, corrupted samples and then distills it into a one-step generator capable of producing refined, clean outputs. While score distillation is traditionally viewed as a method to accelerate diffusion models, we show that it can also significantly enhance sample quality, particularly when starting from a degraded teacher model. Across varying noise levels and datasets, DSD consistently improves generative performancewe summarize our empirical evidence in Fig. 1. Furthermore, we provide theoretical insights showing that, in a linear model setting, DSD identifies the eigenspace of the clean data distributions covariance matrix, implicitly regularizing the generator. This perspective reframes score distillation as not only a tool for efficiency but also a mechanism for improving generative models, particularly in low-quality data settings.

==> preamble.tex <==
%
% --- inline annotations
%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/auxillary_proof.tex <==


\subsection{Proof of Theorem \ref{thm:r=1}}


% We will consider the following setup for our theoretical analysis: suppose our underlying data distribution is given by a low-rank linear model of the form $x = Ez \sim p_X$ where $z \sim \cN(0,I_r)$ where $E \in \RR^{d \times r}$ with $r < d$ and $E$ has orthonormal columns. We will consider the $r=1$ case for simplicity. Then the data distribution $p_X$  degenerate Gaussian of the form $$p_X := \cN(0,e_1e_1^T),$$ where $e_1 \in \RR^d$ is the first standard basis vector in $\RR^d$ (any arbitrary unit vector would suffice). For a fixed noise level $\sigma > 0$, suppose we only have access to the noisy distribution $$y = x+ \sigma z,\ z \sim \cN(0,I_d) \Longleftrightarrow p_{Y,\sigma} := \cN(0,e_1e_1^T + \sigma^2 I_d).$$ Given this distribution, we will assume we have perfectly learned the score $$s_{\sigma}(x):= \nabla \log p_{Y,\sigma}(x) = - (e_1e_1^T + \sigma^2 I_d)^{-1}x.$$ Our goal is to distill this distribution into a distribution $p_{G_{\theta}} := (G_{\theta})_{\sharp}(\cN(0,I_d))$ given by the push-forward of Gaussian $\cN(0,I_d)$ induced by a generative neural network $G_{\theta} : \RR^d \rightarrow \RR^d$. This will be done by minimizing the score-based loss (or Fisher divergence) as in \cite{zhou2024score}: \begin{align*}
% \cL(\theta) := \EE_{x \sim p_G}\left[\|s_{\sigma}(x) - \nabla \log p_{G_{\theta}}(x)\|_2^2\right].  
% \end{align*} To model the U-Net \cite{ronneberger2015u} style architecture with low-rank structure, we will consider maps $G_{\theta}$ with $\theta = (u,v)$ of the form $$G_{\theta}(z) := uv^Tz\ \text{where}\ \theta=(u,v):  \|u\|_2 = 1, v \in \RR^d. $$
% Let $\mathbb{S}^{d-1} := \{u \in \RR^d : \|u\|_2 = 1\}$ denote the unit sphere in $\RR^d$. Consider the constraint set of parameters \begin{align*}
%     \Theta := \{\theta = (u,v) : (u,v) \in \mathbb{S}^{d-1}\times \RR^d\}.
% \end{align*} The following Theorem shows that minimizers of \eqref{eq:ideal-score-loss} induce low-rank distributions that have lower Wasserstein-2 distance to the true distribution than the noisy distribution. We also precisely quantify how far these distributions are:
% \begin{theorem}
%     Fix $\sigma > 0$. Consider the distributions $p_X := \cN(0,e_1e_1^T)$ and $p_{Y,\sigma} := \cN(0,e_1e_2^T + \sigma^2I_d)$. Then the global minimizers of \eqref{eq:ideal-score-loss} over the constraint set $\theta_* \in \Theta$ are precisely either \begin{align}
%         & (u_*,v_*) : u_*=e_1\ \text{and}\ \|v_*\|_2 = \sqrt{1+\sigma^2}\  \label{eq:case1} \\
%        \text{or}\ & (u_*,v_*) : u_*=e_i\ \text{and}\ \|v_*\|_2 = \sigma^2\ \text{for any}\ i = 2,\dots,d \label{eq:case2}.
%     \end{align} For a global minimizer $\theta_*$, consider the induced distilled distribution $p_{G_{\theta_*}}.$ If $\theta_*$ satisfies \eqref{eq:case1}, then for any $d \in \mathbb{N}$, $$W_2^2(p_{G_{\theta_*}},p_X)
%          = W_2^2(p_{Y,\sigma},p_X) - (d-1)\sigma^2.$$ Otherwise, if $\theta_*$ satisfies \eqref{eq:case2}, then if $$d > 1 - \frac{1 + 2\sqrt{1+\sigma^2}(\sigma - 1)}{\sigma^2},$$ we have \begin{align*}
%               W_2^2(p_{G_{\theta_*}},p_X) < W_2^2(p_{Y,\sigma},p_X).
%          \end{align*} Note that this condition on $d$ is trivially satisfied if $\sigma \geqslant 1$.
% \end{theorem}

 
    % Observe that for $\theta = (u,v)$, the induced distribution is $$p_{G_{\theta}} = \cN(0,\|v\|_2^2 uu^T).$$ Note that the score function of $p_{G_{\theta}}$ is well-defined on $\mathrm{span}(u)$ and is given by \begin{align*}
    %     \nabla \log p_{G_{\theta}}(x) = - (\|v\|_2^2uu^T)^{\dagger}x = -\|v\|_2^{-2}uu^Tx.
    % \end{align*} We now simplify the loss function $\cL:$ for $\theta$ such that $\|u\|_2 = 1$, we have
    % \begin{align*}
    %    & \cL(\theta)  = \EE_{x \sim p_G}\left[\|s_{\sigma}(x) - \nabla \log p_{G_{\theta}}(x)\|_2^2\right] \\
    %     & = \EE_{x \sim p_G}\left[\|(e_1e_1^T + \sigma^2 I_d)^{-1}x - \|v\|_2^{-2}uu^Tx\|_2^2\right] \\
    %     & = \EE_{z \sim \cN(0,I_d)}\left[\|(e_1e_1^T + \sigma^2 I_d)^{-1}uv^Tz - \|v\|_2^{-2}uu^Tuv^Tz\|_2^2\right] \\
    %     & = \EE_{z \sim \cN(0,I_d)}\left[v^Tz\right]\cdot\|(e_1e_1^T + \sigma^2 I_d)^{-1}u - \|v\|_2^{-2}u\|_2^2 \\
    %     & = \|v\|_2^2\cdot\|(e_1e_1^T + \sigma^2 I_d)^{-1}u - \|v\|_2^{-2}u\|_2^2
    % \end{align*} where we used $\|u\|_2 = 1$ in the fourth equality and the fact that $v^Tz \sim \cN(0,\|v\|_2^2)$ for $z \sim \cN(0,I_d)$ in the final equality. Thus, in order to minimize this loss we must have that \begin{align*}
    %     (e_1e_1^T + \sigma^2 I_d)^{-1}u = \|v\|_2^{-2}u.
    % \end{align*} That is, $(u,\|v\|_2^{-2})$ must be an eigenpair of the matrix $(e_1e_1^T + \sigma^2 I_d)^{-1}.$
   By Lemma \ref{lemma2},  the distance between the noisy distribution $p_{Y,\sigma}$ and the data distribution $p_X$ is given by \begin{align*}
        W_2^2(p_{Y,\sigma},p_X) = 2+\sigma^2 -2\sqrt{1+\sigma^2} + (d-1)\sigma^2.
    \end{align*} 
    % We then try to find the global minimizes of \eqref{eq:ideal-score-loss-r} and calculate $W_2^2(p_{G_{\theta_*}},p_X)$.
    
     Observe that for $\theta = (u,v)$, the induced distribution is $p_{G_{\theta}} = \cN(0,\|v\|_2^2 uu^T).$ Note that the score function of $p_{G_{\theta}}$ is well-defined on $\mathrm{span}(u)$ and is given by $
        \nabla \log p_{G_{\theta}}(x)= -\|v\|_2^{-2}uu^Tx.$ We now simplify the loss function (\ref{eq:ideal-score-loss-r}):  for $\theta$ such that $\|u\|_2 = 1$, we have
    \begin{align*}
       & \cL(\theta)  = \EE_{x \sim p_G}\left[\|s_{\sigma}(x) - \nabla \log p_{G_{\theta}}(x)\|_2^2\right] \\
        & = \EE_{x \sim p_G}\left[\|(e_1e_1^T + \sigma^2 I_d)^{-1}x - \|v\|_2^{-2}uu^Tx\|_2^2\right] \\
        & = \EE_{z \sim \cN(0,I_d)}\left[\|(e_1e_1^T + \sigma^2 I_d)^{-1}uv^Tz - \|v\|_2^{-2}uu^Tuv^Tz\|_2^2\right] \\
        & = \EE_{z \sim \cN(0,I_d)}\left[v^Tz\right]\cdot\|(e_1e_1^T + \sigma^2 I_d)^{-1}u - \|v\|_2^{-2}u\|_2^2 \\
        & = \|v\|_2^2\cdot\|(e_1e_1^T + \sigma^2 I_d)^{-1}u - \|v\|_2^{-2}u\|_2^2,
    \end{align*} where we used $\|u\|_2 = 1$ in the fourth equality and the fact that $v^Tz \sim \cN(0,\|v\|_2^2)$ for $z \sim \cN(0,I_d)$ in the final equality. Thus, in order to minimize this loss we must have that \begin{align*}
        (e_1e_1^T + \sigma^2 I_d)^{-1}u = \|v\|_2^{-2}u.
    \end{align*} That is, $(u,\|v\|_2^{-2})$ must be an eigenpair of the matrix $(e_1e_1^T + \sigma^2 I_d)^{-1}.$ 
    Note that this matrix has the following pairs of eigenvectors and eigenvalues: $$(e_1,(1+\sigma^2)^{-1})\ \text{and}\ (e_i,\sigma^{-2})\ \forall i =2,\dots,d$$ where $e_i$ is the $i$-th standard basis vector. Thus, the global minimizers   $\theta^* = (u_*,v_*)$   must satisfy $$u_*=e_1,\|v_*\|_2=\sqrt{1+\sigma^2}\ \text{or}\ u_*=e_i,\|v_*\|_2=\sigma.$$

    We will consider the following cases:
    \paragraph{Top eigenpair:} Suppose $u_* = e_1$ and $v_*$ satisfies $\|v_*\|_2 = \sqrt{1+\sigma^2}$. Then $$p_{G_{\theta_*}} = \cN(0,(1+\sigma^2)e_1e_1^T).$$ By Lemma \ref{lemma2}, we now compute \begin{align*}
        W_2^2(p_{G_{\theta_*}},p_X) & = 2+\sigma^2 - 2\sqrt{1+\sigma^2}. \end{align*}
As a result,     
     $$W_2^2(p_{G_{\theta_*}},p_X)
         = W_2^2(p_{Y,\sigma},p_X) - (d-1)\sigma^2 <  W_2^2(p_{Y,\sigma},p_X).$$ 


    \paragraph{Lower eigenpair:} Suppose $u_* = e_i$ for some $i =2,\dots,d$ and $\|v_*\|_2 = \sigma.$ Then \begin{align*}
    p_{G_{\theta_*}} = \cN(0,\sigma^2e_ie_i^T).
    \end{align*} 
   \ys{The original result is wrong. I recompute it, please verify:} By Lemma \ref{lemma2}, we now compute 
    \begin{align*}
        W_2^2(p_{G_{\theta_*}},p_X) & = 1 + \sigma^2 - 2 \sigma. \end{align*}
    A simple rearranging shows that the condition on $d$ is equivalent to the following: \begin{align*}
        1 + \sigma^2 - 2\sigma< 2 + \sigma^2 - 2\sqrt{1+\sigma^2} + (d-1)\sigma^2 \Longleftrightarrow d > 1 + \frac{2(\sqrt{1+\sigma^2}-\sigma)-1}{\sigma^2}.
    \end{align*} Hence by calculating the Wasserstein distance, we see that by assumption on $d$, \begin{align*}
        W_2^2(p_{G_{\theta_*}},p_X) & = 1 + \sigma^2 - 2\sigma \\
        & < 2 + \sigma^2 - 2\sqrt{1+\sigma^2} + (d-1)\sigma^2 \\
        & = W_2^2(p_{Y,\sigma},p_X)
    \end{align*} as desired.

    \ys{Do we need to compare the real distance under the two different cases? i.e. compare $2+\sigma^2 - 2\sqrt{1+\sigma^2}$ and $1 + \sigma^2 - 2\sigma$? Similar results are in my proof for general $r$. Let's do a difference. Define $g(\sigma) =1-2\sqrt{1+\sigma^2} +2\sigma$, which is an increasing function when $\sigma > 0.$ 
When $\sigma < 3/4$, $g(\sigma) <0$. In this case, choose the top eigenpair.
In contrast, when $\sigma > 3/4$, $g(\sigma) >0$. In this case, choose the lower eigenpair.
However, we have that for any $\sigma >0$ and any $d \in \NN$, choosing the top eigenpair  is sufficient to ensure that  $
W_2^2(p_{G_{\theta^*}},p_X) < W_2^2(p_{Y,\sigma},p_X)$ holds.  }

\ys{My conclusion is when $\sigma < 3/4$, choose the top eigenpair. When $\sigma > 3/4$, choose the lower eigenpaier. In this case $h(\sigma) < h(3/4) = 1$ because $h(\sigma)$ is an decreasing function when $\sigma < 3/4$. (see the definition of $h$ below), the condition $d > h(\sigma)$ is naturally satisfied.  }

\begin{remark}
    As for the lower eigenpair case, denote $h(\sigma) =1 + \frac{2(\sqrt{1+\sigma^2}-\sigma)-1}{\sigma^2} = 1 + \frac{2}{\sigma}(\sqrt{\frac{1}{\sigma^2}+1}-1)-\frac{1}{\sigma^2} $. Let $k = \frac{1}{\sigma}$. Then $h(k) = 1 + 2k(\sqrt{k^2+1}-1) - k^2$. When $\sigma$ goes to infinity, i.e., $k$ goes to 0, $h(\sigma)$ approximates 0. In this case, the assumption on $d$ is easy to satisfy. On the other hand,  when $\sigma$ goes to 0, i.e. $k$ goes to infinity, $h(\sigma)$ will go to infinity. In this case, the assumption on $d$ becomes increasingly difficult to satisfy. However, our scenario remains well-suited for noisy data with a non-trivial level of $\sigma$. 
\end{remark}

\begin{remark}
  We note that the top eigenpair case produces better distilled student models for any $d \in \NN$. In this sense, lower eigenpairs act as local minimizers, whereas the top eigenpair corresponds to a global minimizer. If global optimize[rs are guaranteed, distilled models can consistently outperform teacher models without any additional conditions. 
\end{remark}

% \subsection{Note on ambient score matching objective}

 
% I have a question, if 
% \begin{align}
%     y = x + \sigma z, ~ z \sim \cN(0,1)
% \end{align}
% Assume we know $x$ is normal, then $y$ is normal. if we can learn/measure
% \begin{align}
%     y \sim \cN(0, \sigma_y^2I),
% \end{align}
% can we say something about the distribution of $x$?
% Note that by tweedie's formula, we have the expectation $\EE(x|y)$, this is useless when the means are all zero. 

% We in fact can get the \begin{align}
%     \sigma_x^2 = \sigma_y^2 - \sigma^2.
% \end{align}
% In some sense, in the toy example, the diffusion models can have \textbf{perfect estimation of the clean data distribution.}

% Then, how about the real case? I think we may need to consider the approximation/discretization error. This will complicate the proof quite a lot. 

% Let's think that when $x$ is no longer normal, $y$ is an unknown distribution,  we still have 
% \begin{align}
%      \sigma_x^2 = \sigma_y^2 - \sigma^2.
% \end{align}
% but \textbf{this is not useful }cause the variance contains very little information when we have a complicated image data distribution of $x$. 

\subsection{Proof of Theorem \ref{thm:general-r}}

%We now extend our analysis to the general rank \(r\). 
% Suppose our underlying data distribution is given by a low-rank linear model
% \[
% x = Ez \sim p_X, \quad z \sim \mathcal{N}(0,I_r),
% \]
% where \(E \in \mathbb{R}^{d \times r}\) with \(r < d\) and with orthonormal columns (i.e. \(E^TE=I_r\)). Then, 
% \[
% p_X := \mathcal{N}(0,EE^T).
% \]
% For a fixed noise level \(\sigma > 0\), suppose we only have access to the noisy distribution
% \[
% y = x + \sigma z, \quad z \sim \mathcal{N}(0,I_d) \quad \Longleftrightarrow \quad p_{Y,\sigma} := \mathcal{N}(0,EE^T+\sigma^2 I_d).
% \]
% Given this distribution, we assume that we have perfectly learned the score
% \[
% s_\sigma(x) := \nabla \log p_{Y,\sigma}(x) = -\bigl(EE^T+\sigma^2I_d\bigr)^{-1}x.
% \]
% Our goal is to distill this distribution into a distribution 
% \[
% p_{G_\theta} := (G_\theta)_\sharp \mathcal{N}(0,I_d)
% \]
% given by the push-forward of \(\mathcal{N}(0,I_d)\) by a generative network \(G_\theta : \mathbb{R}^d \to \mathbb{R}^d\). To model a U-Net style architecture with low-rank structure, we consider maps \(G_\theta\) with \(\theta = (U,V)\) of the form
% \[
% G_\theta(z) := U V^T z,
% \]
% where
% \[
% U \in \mathbb{R}^{d \times r} \quad \text{with} \quad U^TU=I_r \quad \text{and} \quad V \in \mathbb{R}^{d \times r}.
% \]
% Let
% \[
% \Theta := \{(U,V): U \in \mathrm{St}(d,r),\, V \in \mathbb{R}^{d\times r}\}.
% \]
% We then distill the noisy distribution by minimizing the score-based loss (or Fisher divergence)
% \begin{equation}\label{eq:ideal-score-loss}
% \mathcal{L}(\theta) := \mathbb{E}_{x\sim p_{G_\theta}}\left[\|s_\sigma(x)-\nabla\log p_{G_\theta}(x)\|_2^2\right].
% \end{equation}

% \begin{theorem}[General Rank \(r\)]
% Fix \(\sigma>0\). Then the global minimizers of \eqref{eq:ideal-score-loss} over \(\Theta\) are precisely those \(\theta=(U,V)\) satisfying
% \[
% U^T\bigl(EE^T+\sigma^2I_d\bigr)^{-1}U = (V^TV)^{-1}.
% \]
% In particular, one set of global minimizers is given by
% \begin{equation}\label{eq:good-case}
% U = E \quad (\text{up to an orthogonal transformation}) \quad \text{and} \quad V^TV = (1+\sigma^2)I_r,
% \end{equation}
% which induces the distilled distribution
% \[
% p_{G_{\theta^*}} = \mathcal{N}(0,(1+\sigma^2)EE^T).
% \]
% Moreover, one can verify that
% \[
% W_2^2(p_{G_{\theta^*}},p_X) = W_2^2(p_{Y,\sigma},p_X) - (d-r)\sigma^2 < W_2^2(p_{Y,\sigma},p_X).
% \]
% \end{theorem}

Observe that for \(\theta=(U,V)\), the induced distribution is
\[
p_{G_\theta} = \mathcal{N}(0, U(V^TV)U^T).
\]
Note that the score function of \(p_{G_\theta}\) is well-defined on the subspace \(\mathrm{range}(U)\) and is given by
\[
\nabla\log p_{G_\theta}(x) = -\Bigl(U(V^TV)U^T\Bigr)^{\dagger}x = -U(V^TV)^{\dagger}U^Tx.
\]
We now simplify the loss function \(\mathcal{L}(\theta)\) in \eqref{eq:ideal-score-loss-r}: 
\[
\begin{aligned}
\mathcal{L}(\theta) &= \mathbb{E}_{x\sim p_{G_\theta}}\Bigl[\Bigl\|\bigl(EE^T+\sigma^2I_d\bigr)^{-1}x - U(V^TV)^{\dagger}U^Tx\Bigr\|_2^2\Bigr] \\
 &= \mathbb{E}_{z\sim \cN(0, I_d)}\Bigl[\Bigl\|\bigl(EE^T+\sigma^2I_d\bigr)^{-1}UV^Tz - U(V^TV)^{\dagger}U^TUV^Tz\Bigr\|_2^2\Bigr] \\
&= \mathbb{E}_{y\sim \mathcal{N}(0,V^TV)}\Bigl[\Bigl\|\Bigl((EE^T+\sigma^2I_d)^{-1}U - U(V^TV)^{\dagger}\Bigr)y\Bigr\|_2^2\Bigr]. & \text{\# Define $y = V^Tz$.} 
\end{aligned}
\]
Define the matrix $
A := (EE^T+\sigma^2I_d)^{-1}U.
$
Then, we can write
\[
\mathcal{L}(\theta) = \mathbb{E}_{y\sim \mathcal{N}(0,V^TV)}\| (A-U(V^TV)^{\dagger})y\|_2^2.
\]
Express the squared norm as a quadratic form:
\[
\| (A-U(V^TV)^{-1})y\|_2^2 = y^T\Bigl[ \bigl(A-U(V^TV)^{\dagger}\bigr)^T\bigl(A-U(V^TV)^{\dagger}\bigr)\Bigr]y.
\]
Using the property that for \(y\sim \mathcal{N}(0,V^TV)\), we have \(\mathbb{E}[yy^T]=V^TV\). Then, the loss function can be simplified as 
\[
\mathcal{L}(\theta) = \operatorname{Tr}\Bigl[\bigl(A-U(V^TV)^{\dagger}\bigr)^T\bigl(A-U(V^TV)^{\dagger}\bigr) (V^TV)\Bigr].
\]
As a result, \(\mathcal{L}(\theta)=0\) (i.e. the loss is minimized) if and only if
$$
A = U(V^TV)^{\dagger},$$
{or equivalently}, 
\begin{align*}
    (EE^T+\sigma^2I_d)^{-1}U = U(V^TV)^{\dagger}.
\end{align*}

By Lemma \ref{lemma1}, we have $$(EE^T + \sigma^2 I_d)^{-1} = \sigma^{-2}I_d - (\sigma^2(\sigma^2+1))^{-1}EE^T.$$ 
Hence, our main condition reads 
\begin{align}\label{eq:main-eq}
    \left[\sigma^{-2}I_d - (\sigma^2(\sigma^2+1))^{-1}EE^T\right]U = U(V^TV)^{\dagger}.
\end{align}
We first note that the matrix $\sigma^{-2}I_d - (\sigma^2(\sigma^2+1))^{-1}EE^T$ has eigenvectors either in $\mathrm{col}(E)$ with eigenvalue $(\sigma^2(\sigma^2+1))^{-1}$ or in $\mathrm{col}(E)^{\perp}$ with eigenvalue $\sigma^{-2}.$

The right-hand side of \eqref{eq:main-eq} implies that anything on the left must lie in the column span of $U$.   In order for $\left[\sigma^{-2}I_d - (\sigma^2(\sigma^2+1))^{-1}EE^T\right]U$ to continue to lie in the column span of $U$, we must have that the columns of $U$ either lie in $\mathrm{col}(E)$ or $\mathrm{col}(E)^{\perp}$. That is, of the $r$ columns $u_1,\dots,u_r$, we can have $k\leqslant r$ columns in $\mathrm{col}(E)$ and $r-k$ columns in $\mathrm{col}(E)^{\perp}$. Partition $U = [U_1\  U_2]$ where $U_1 \in \mathbb{R}^{d \times k}$ and $U_2 \in \mathbb{R}^{d \times (r-k)}$ with $\mathrm{col}(U_1) \subseteq \mathrm{col}(E)$ and $\mathrm{col}(U_2) \subseteq \mathrm{col}(E)^{\perp}$. This always holds up to reordering of the columns. Then, we have $EE^T U_1 = U_1$ and $EE^T U_2 = 0$. Thus, with this notation, we get \begin{align*}
    \left(\sigma^{-2}I_d - (\sigma^2(\sigma^2+1))^{-1}EE^T\right)U & = \left(\sigma^{-2}I_d - (\sigma^2(\sigma^2+1))^{-1}EE^T\right)[U_1\ U_2] \\
    & = \left[\sigma^{-2}U_1 - (\sigma^2(\sigma^2+1))^{-1}U_1,\ \sigma^{-2}U_2 \right] \\
    & = \left[(\sigma^2+1)^{-1}U_1,\ \sigma^{-2}U_2\right] \\
    & = [U_1\ U_2] \left[\begin{array}{cc}
        (\sigma^2+1)^{-1}I_{k} & 0  \\
        0 & \sigma^{-2}I_{r-k}
    \end{array}\right] \\
    & = U \left[\begin{array}{cc}
        (\sigma^2+1)^{-1}I_{k} & 0  \\
        0 & \sigma^{-2}I_{r-k}
    \end{array}\right].
\end{align*} Hence our final equation reads: \begin{align*}
   & \left(\sigma^{-2}I_d - (\sigma^2(\sigma^2+1))^{-1}EE^T\right)U = U(V^TV)^{\dagger} \\
   \Longleftrightarrow\ & U \left[\begin{array}{cc}
        (\sigma^2+1)^{-1}I_{k} & 0  \\
        0 & \sigma^{-2}I_{r-k}
    \end{array}\right]= U(V^TV)^{\dagger}.
\end{align*} 
%Note that this is similar to the final result you get, but now this allows for the situation where the columns of $U$ have some of the eigenvectors of $E$ ($k$ of them) and some of the eigenvectors in the orthogonal complement ($r-k$ of them). This is the full characterization of possible minimizers.

As a result, the possible solutions are: $(U,V)$ such that \begin{align*}
    & U = [U_1\ U_2],\ U_1 \in \mathbb{R}^{d \times k},\ U_2 \in \mathbb{R}^{d\times (r-k)}\ (\text{up to column reordering})\ \text{such that} \\
    & \mathrm{col}(U_1) \subseteq \mathrm{col}(E),\ \mathrm{col}(U_2) \subseteq \mathrm{col}(E)^{\perp}\ \text{and} \\
    & V^TV = \left[\begin{array}{cc}
        (\sigma^2+1)I_{k} & 0  \\
        0 & \sigma^{2}I_{r-k}
    \end{array}\right].
    \end{align*} Note that the last condition on $V$ means that the first $k$ columns of $V$ are mutually orthogonal with norm $\sqrt{\sigma^2+1}$ and the final $r-k$ columns are mutually orthogonal with norm $\sigma$.

    Next, we start to compute the Wasserstein-2 distance. By Lemma \ref{lemma2}, we have
    \[
\begin{aligned}
W_2^2(p_{Y,\sigma},p_X) &= r\Bigl((1+\sigma^2)+1-2\sqrt{1+\sigma^2}\Bigr) + (d-r)\sigma^2,\\
W_2^2(p_{G_{\theta^*}},p_X) &= k\Bigl((1+\sigma^2)+1-2\sqrt{1+\sigma^2}\Bigr) + (r-k)(1 + \sigma^2-2\sigma) \\
&= r(1+\sigma^2-2\sigma)  +k\Bigr(1-2\sqrt{1+\sigma^2} +2\sigma\Bigr).
\end{aligned}
\]

Define $g(\sigma) =1-2\sqrt{1+\sigma^2} +2\sigma$, which is an increasing function when $\sigma > 0.$ 
When $\sigma < 3/4$, $g(\sigma) <0$. In this case, choosing $k=r$ yields the smallest distance. 
In contrast, when $\sigma > 3/4$, $g(\sigma) >0$. In this case, choosing $k=0$ yields the smallest distance. 

Next, we show that for any $\sigma >0$, choosing $k=r$  is sufficient to ensure that  $
W_2^2(p_{G_{\theta^*}},p_X) < W_2^2(p_{Y,\sigma},p_X)$ hold. 

\ys{define $h(\sigma) = r + \frac{r\Bigl(2(\sqrt{1+\sigma^2}-\sigma)-1\Bigr)}{\sigma^2}$.}

    \ys{My conclusion is when $\sigma < 3/4$, choose $k=r$. When $\sigma > 3/4$, choose the $k=0$. In this case $h(\sigma) < h(3/4) = r$ because $h(\sigma)$ is an decreasing function when $\sigma < 3/4$. (see the definition of $h$ below), the condition $d > h(\sigma)$ is naturally satisfied.  }











\paragraph{Optimal Case.} When $k=r$, one can compute
\[
\begin{aligned}
W_2^2(p_{G_{\theta^*}},p_X) &= r\Bigl((1+\sigma^2)+1-2\sqrt{1+\sigma^2}\Bigr).
\end{aligned}
\]
Hence, for any $d \in \NN$, 
\[
W_2^2(p_{G_{\theta^*}},p_X) = W_2^2(p_{Y,\sigma},p_X)-(d-r)\sigma^2 < W_2^2(p_{Y,\sigma},p_X),
\]
as desired.


\textbf{Suboptimal Case.} When $k=0$, one can compute
\[
W_2^2(p_{G_\theta},p_X)= r\Bigl(1+\sigma^2-2\sigma\Bigr).
\]
A short calculation shows that if
\[
d >  r + \frac{r\Bigl(2(\sqrt{1+\sigma^2}-\sigma)-1\Bigr)}{\sigma^2},
\]
then
\[
W_2^2(p_{G_\theta},p_X) < W_2^2(p_{Y,\sigma},p_X).
\]

\begin{remark}
    
\end{remark}

==> sec/old_theory.tex <==
\subsection{Proof of Theorem \ref{thm:epsilon-theorem}} \label{sec:appx-theorem-proof}
\paragraph{Reduction of objective function:} For notational convenience, set $\Sigma_{\varepsilon} := UV^TVU^T + \varepsilon^2 I_d$ and $\Sigma_{\sigma} := EE^T + \sigma^2 I_d$, so that $s_{\sigma}(x) = -\Sigma_{\sigma}^{-1}x$ and $\nabla \log p^{\varepsilon}_{G_{\theta}}(x) = -\Sigma_{\varepsilon}^{-1}x$. First, recall that for $x \sim p^{\varepsilon}_{G_{\theta}}$ and any matrix $\Sigma$, we have $\mathbb{E}_{x \sim p^{\varepsilon}_{G_{\theta}}}[\|\Sigma x\|_2^2] = \mathbb{E}_{z \sim \mathcal{N}(0,I_d)}[\|\Sigma \Sigma_{\varepsilon}^{1/2}z\|_2^2] = \|\Sigma \Sigma_{\varepsilon}^{1/2}\|_F^2.$ Using this, we can compute the loss as follows: \begin{align*}
    \mathcal{L}_{\varepsilon}(\theta) & = \mathbb{E}_{x \sim p^{\varepsilon}_{G_{\theta}}}\left[\|(\Sigma_{\sigma}^{-1} - \Sigma_{\varepsilon}^{-1})x\|_2^2\right] \\
    & = \|(\Sigma_{\sigma}^{-1} - \Sigma_{\varepsilon}^{-1})\Sigma_{\varepsilon}^{1/2}\|_F^2 \\
    & = \mathrm{tr}\left(\Sigma_{\varepsilon}^{1/2}(\Sigma_{\sigma}^{-1} - \Sigma_{\varepsilon}^{-1}) (\Sigma_{\sigma}^{-1} - \Sigma_{\varepsilon}^{-1})\Sigma_{\varepsilon}^{1/2}\right) \\
    & = \mathrm{tr}\left(\Sigma_{\varepsilon}(\Sigma_{\sigma}^{-1} - \Sigma_{\varepsilon}^{-1}) (\Sigma_{\sigma}^{-1} - \Sigma_{\varepsilon}^{-1})\right)\\
    & = \mathrm{tr}\left((\Sigma_{\varepsilon}\Sigma_{\sigma}^{-1} - I_d) (\Sigma_{\sigma}^{-1} - \Sigma_{\varepsilon}^{-1})\right) \\
    & = \mathrm{tr}\left(\Sigma_{\varepsilon}\Sigma_{\sigma}^{-2} -\Sigma_{\varepsilon}\Sigma_{\sigma}^{-1}\Sigma_{\varepsilon}^{-1} - \Sigma_{\sigma}^{-1} + \Sigma_{\varepsilon}^{-1}\right) \\
    & = \mathrm{tr}\left(\Sigma_{\varepsilon}\Sigma_{\sigma}^{-2}\right) -\mathrm{tr}\left(\Sigma_{\varepsilon}\Sigma_{\sigma}^{-1}\Sigma_{\varepsilon}^{-1}\right) - \mathrm{tr}\left(\Sigma_{\sigma}^{-1}\right) + \mathrm{tr}\left(\Sigma_{\varepsilon}^{-1}\right) \\
    & = \mathrm{tr}\left(\Sigma_{\sigma}^{-2}\Sigma_{\varepsilon}\right) - 2\mathrm{tr}\left(\Sigma_{\sigma}^{-1}\right) + \mathrm{tr}\left(\Sigma_{\varepsilon}^{-1}\right) \\
    & =: C_{\sigma} + \mathrm{tr}\left(\Sigma_{\sigma}^{-2}\Sigma_{\varepsilon}\right) +\mathrm{tr}\left(\Sigma_{\varepsilon}^{-1}\right).
\end{align*} Using Lemma \ref{lemma2}, it is straightforward to see that \begin{align*}
    \Sigma_{\sigma}^{-1} = \frac{1}{\sigma^2} I_d - \frac{1}{\sigma^2(\sigma^2+1)}EE^T\ \text{and}\ \Sigma_{\varepsilon}^{-1} = \varepsilon^{-2}I_d - \varepsilon^{-4}U\left((V^TV)^{-1} + \varepsilon^{-2}I_r\right)^{-1}U^T
\end{align*} Hence the third term in $\mathcal{L}_{\varepsilon}$ is given by $$\mathrm{tr}(\Sigma_{\varepsilon}^{-1}) = \mathrm{tr}\left(\varepsilon^{-2}I_d - \varepsilon^{-4}U\left((V^TV)^{-1} + \varepsilon^{-2}I_r\right)^{-1}U^T\right) =: C_{\varepsilon} - \varepsilon^{-4}\mathrm{tr}\left(\left((V^TV)^{-1} + \varepsilon^{-2}I_r\right)^{-1}\right)$$ where we used the cyclic property of the trace and $U^TU=I_r$ in the last equality. For the second term, let $\gamma_{\sigma}:= 1/(\sigma^2(\sigma^2+1))$. For the second term, we have by direct computation, \begin{align*}
    \mathrm{tr}\left(\Sigma_{\sigma}^{-2}\Sigma_{\varepsilon}\right) & = \mathrm{tr}\left(\left(\sigma^{-2}I_d - \gamma_{\sigma}EE^T\right)\left(\sigma^{-2}I_d - \gamma_{\sigma}EE^T\right) (UV^TVU^T+\varepsilon^2I_d)\right) \\
    & = \mathrm{tr}\left(\left(\sigma^{-4}I_d - 2\sigma^{-2}\gamma_{\sigma}EE^T + \gamma_{\sigma}^2EE^T\right) (UV^TVU^T+\varepsilon^2I_d)\right) \\
    & = \mathrm{tr}\left(\sigma^{-4}UV^TVU^T - \varepsilon^2\sigma^{-4}I_d +\left(\gamma_{\sigma}^2 - 2\sigma^{-2}\gamma_{\sigma}\right) \gamma_{\sigma}EE^TUV^TVU^T - 2\sigma^{-2}\varepsilon^2\gamma_{\sigma}EE^T + \gamma_{\sigma}^2\varepsilon^2I_d\right) \\
    & =:\Tilde{C}_{\sigma,\varepsilon} + \sigma^{-4}\mathrm{tr}(UV^TVU^T) +\left(\gamma_{\sigma}^2 - 2\sigma^{-2}\gamma_{\sigma}\right) \cdot \mathrm{tr}(EE^TUV^TVU^T) \\
    & = \Tilde{C}_{\sigma,\varepsilon} + \sigma^{-4}\mathrm{tr}(V^TV) +\left(\gamma_{\sigma}^2 - 2\sigma^{-2}\gamma_{\sigma}\right) \cdot \mathrm{tr}(EE^TUV^TVU^T)
    \end{align*} where we used the cyclic property of trace and orthogonality of $U$ in the final line. Combining the above displays, we get that there exists a constant $C_{\sigma,\varepsilon} := C_{\sigma} + C_{\varepsilon} + \Tilde{C}_{\sigma,\varepsilon}$ such that \begin{align*}
        \mathcal{L}_{\varepsilon}(\theta) & = C_{\sigma,\varepsilon} + \left(\frac{1}{\sigma^4(\sigma^2+1)^2} - \frac{2}{\sigma^4(\sigma^2+1)}\right)\cdot\mathrm{tr}(EE^TUV^TVU^T) \\
        & + \sigma^{-4}\mathrm{tr}(V^TV) - \varepsilon^{-4}\mathrm{tr}\left(\left((V^TV)^{-1} + \varepsilon^{-2}I_r\right)^{-1}\right) \\
        & =: C_{\sigma,\varepsilon} + B(U,V) + R(V)
    \end{align*} where we have defined the quantities \begin{align*}
        B(U,V) & := \underbrace{\left(\frac{1}{\sigma^4(\sigma^2+1)^2} - \frac{2}{\sigma^4(\sigma^2+1)}\right)}_{< 0}\cdot\mathrm{tr}(EE^TUV^TVU^T)\ \text{and} \\
        R(V) & := \sigma^{-4}\mathrm{tr}(V^TV) -\varepsilon^{-4}\mathrm{tr}\left(\left((V^TV)^{-1} + \varepsilon^{-2}I_r\right)^{-1}\right).
    \end{align*} Hence we have the equivalence $$\argmin_{\theta \in \Theta} \mathcal{L}_{\varepsilon}(\theta) = \argmin_{\theta \in \Theta} B(U,V) + R(V).$$
    
    \paragraph{Form of minimizers:} We first note that we can first minimize $B(U,V)$ over feasible $U$. Due to the negative constant in $B(U,V)$, this is equivalent to maximizing $\mathrm{tr}(EE^TUV^TVU^T).$ Taking $\Sigma = V^TV$ in Lemma \ref{lem:pca-like-result}, we have that the minimizer of $B(U,V)$, for any invertible $V$, is given by $$U^* = EQ\ \text{for some rotation}\ Q.$$ Moreover, the proof of Lemma \ref{lem:pca-like-result} shows that $\mathrm{tr}(EE^TU^*V^TV(U^*)^T) = \mathrm{tr}(V^TV)$. This gives
    \begin{align*}
        B(U^*,V) & = \left(\frac{1}{\sigma^4(\sigma^2+1)^2} - \frac{2}{\sigma^4(\sigma^2+1)}\right) \mathrm{tr}(V^TV).
    \end{align*} In summary, we now must minimize the following with respect to invertible $V$: \begin{align*}
        B(U^*,V) + R(V) & = \left(\frac{1}{\sigma^4(\sigma^2+1)^2} - \frac{2}{\sigma^4(\sigma^2+1)} + \frac{1}{\sigma^4}\right) \mathrm{tr}(V^TV) - \varepsilon^{-4}\mathrm{tr}\left(\left((V^TV)^{-1} + \varepsilon^{-2}I_r\right)^{-1}\right) \\
        & = \frac{1}{\sigma^4}\left(\frac{1}{\sigma^2 + 1} - 1\right)^2 \mathrm{tr}(V^TV) - \varepsilon^{-4}\mathrm{tr}\left(\left((V^TV)^{-1} + \varepsilon^{-2}I_r\right)^{-1}\right) \\
        & = \frac{1}{\sigma^4}\left(\frac{\sigma^2}{\sigma^2 + 1}\right)^2 \mathrm{tr}(V^TV) - \varepsilon^{-4}\mathrm{tr}\left(\left((V^TV)^{-1} + \varepsilon^{-2}I_r\right)^{-1}\right) \\
        & = \frac{1}{(\sigma^2 + 1)^2} \mathrm{tr}(V^TV) - \varepsilon^{-4}\mathrm{tr}\left(\left((V^TV)^{-1} + \varepsilon^{-2}I_r\right)^{-1}\right)
    \end{align*} where in the second equality, we completed the square.

    We now claim that $B(U^*,V) + R(V)$ solely depends on the eigenvalues of $V^TV$. In particular, for invertible $V$, note that $V^TV \succ 0$ so it admits the decomposition $V^TV = Q\Lambda Q^T$ where $Q^TQ=QQ^T=I_r$ and $\Lambda$ is a diagonal matrix with positive entries $\Lambda_{ii}= \lambda_i(V^TV) > 0$. Hence $\mathrm{tr}(V^TV) = \mathrm{tr}(Q\Lambda Q^T) = \mathrm{tr}(Q^TQ\Lambda)= \mathrm{tr}(\Lambda) = \sum_{i=1}^r \lambda_i(V^TV).$ Likewise, we have using the orthogonality of $Q$ that \begin{align*}
        \mathrm{tr}\left(\left((V^TV)^{-1} + \varepsilon^{-2}I_r\right)^{-1}\right) & = \mathrm{tr}\left(\left((Q\Lambda Q^T)^{-1} + \varepsilon^{-2}I_r\right)^{-1}\right)\\
        & = \mathrm{tr}\left(\left(Q\Lambda ^{-1}Q^T + \varepsilon^{-2}QQ^T\right)^{-1}\right) \\
        & = \mathrm{tr}\left(\left(Q\left(\Lambda^{-1} + \varepsilon^{-2}I_r\right)Q^T\right)^{-1}\right) \\
        & = \mathrm{tr}\left(Q\left(\Lambda^{-1} + \varepsilon^{-2}I_r\right)^{-1}Q^T\right) \\
        & = \mathrm{tr}\left(\left(\Lambda^{-1} + \varepsilon^{-2}I_r\right)^{-1}\right) \\
        & = \sum_{i=1}^r \frac{1}{\lambda_i(V^TV)^{-1} + \varepsilon^{-2}}.
    \end{align*} In sum, the final objective is a particular function of the eigenvalues of $V^TV$: \begin{align*}
        B(U^*,V) + R(V) = \sum_{i=1}^r \left[ \frac{\lambda_i(V^TV)}{(\sigma^2+1)^2} - \frac{1}{\varepsilon^4(\lambda_i(V^TV)^{-1} + \varepsilon^{-2})} \right] =: \sum_{i=1}^r f_{\sigma,\varepsilon}(\lambda_i(V^TV)).
    \end{align*} In Lemma \ref{lem:eigenvalue-function}, we show that when $\varepsilon < \sigma$, the function $t \mapsto f_{\sigma,\varepsilon}(t)$ is strictly convex on $(0,\infty)$ with a unique minimizer when $t = (1+\sigma^2 - \varepsilon^2).$ Thus $V \mapsto B(U^*,V) + R(V)$ for invertible $V$ is minimized when the gram matrix of $V^*_{\varepsilon}$ has equal eigenvalues $\lambda_i((V^*_{\varepsilon})^TV^*_{\varepsilon}) = 1 + \sigma^2 - \varepsilon^2$ for all $i \in [r]$. Since all of its eigenvalues are the same, by the Spectral Theorem, we must have that  $(V^*_{\varepsilon})^TV^*_{\varepsilon} = (1+\sigma^2-\varepsilon^2)I_r.$

    \paragraph{Wasserstein bound:} We now show the Wasserstein error bound. We will first consider the case when $\varepsilon > 0$. We know that $\theta^*_{\varepsilon}$ induces a distribution $$p_{G_{\theta^*_{\varepsilon}}} := \mathcal{N}(0,EQ(1+\sigma^2-\varepsilon^2)I_rQ^TE^T) = \mathcal{N}(0,(1+\sigma^2-\varepsilon^2)EE^T).$$ Then by Lemma \ref{lemma2}, we have
    \[
\begin{aligned}
W_2^2(p_{Y,\sigma},p_X) &= r\Bigl((1+\sigma^2)+1-2\sqrt{1+\sigma^2}\Bigr) + (d-r)\sigma^2,\\
W_2^2(p_{G_{\theta^*_{\varepsilon}}},p_X) &= r\Bigl((1+\sigma^2-\varepsilon^2)+1-2\sqrt{1+\sigma^2-\varepsilon^2}\Bigr).
\end{aligned}
\] Note that \begin{align*}
    W_2^2(p_{G_{\theta^*_{\varepsilon}}},p_X) < W_2^2(p_{Y,\sigma},p_X) & \Longleftrightarrow\\
    2r(\sqrt{1+\sigma^2} - \sqrt{1+\sigma^2-\varepsilon^2}) < (d-r)\sigma^2 + r\varepsilon^2. 
\end{align*} But the sufficient condition $\varepsilon < \sigma \sqrt{\frac{d-r}{r}}$ ensures $2r\varepsilon^2 < (d-r)\sigma^2 + r\varepsilon^2$ which means \begin{align*}
    2r(\sqrt{1+\sigma^2} - \sqrt{1+\sigma^2-\varepsilon^2}) & = 2r\cdot \frac{\varepsilon^2}{\sqrt{1+\sigma^2} + \sqrt{1+\sigma^2-\varepsilon^2}} \\
    & \leqslant 2\varepsilon^2 \\
    & < (d-r)\sigma^2 + r\varepsilon^2
\end{align*} where we used $\sqrt{t} - \sqrt{t -z} = \frac{z}{\sqrt{t} + \sqrt{t-z}}$ for $t > z > 0$ in the first equality and $\sqrt{1+\sigma^2} + \sqrt{1+\sigma^2-\varepsilon^2} \geqslant 1$ in the second inequality. In the limiting case $\theta^* := \lim_{\varepsilon\rightarrow0^+} \theta^*_{\varepsilon}$, we get that $$p_{G_{\theta^*}} := \mathcal{N}(0,(1+\sigma^2)EE^T).$$ This gives $$W_2^2(p_{G_{\theta^*_{\varepsilon}}},p_X) = r\Bigl((1+\sigma^2)+1-2\sqrt{1+\sigma^2}\Bigr).$$ Comparing this to the Wasserstein distance between $p_{Y,\sigma}$ and $p_X$, we see that \begin{align*}
    W_2^2(p_{G_{\theta^*}},p_X) = W_2^2(p_{Y,\sigma},p_X) - (d-r)\sigma^2 < W_2^2(p_{Y,\sigma},p_X) .
\end{align*}



==> sec/theoretical.tex <==
\section{Theory}\label{sec:theory}

We will consider the following linear model setting for our theoretical analysis. Suppose our underlying data distribution is given by a low-rank linear model
$
x = Ez \sim p_X$ and $z \sim \mathcal{N}(0,I_r),
$
where \(E \in \mathbb{R}^{d \times r}\) with \(r < d\) and with orthonormal columns (i.e. \(E^TE=I_r\)). Then, 
$
p_X := \mathcal{N}(0,EE^T).
$
For a fixed noise level \(\sigma > 0\), suppose we only have access to the noisy distribution
$
y = x + \sigma z$, where $z \sim \mathcal{N}(0,I_d)$. In other words, $p_{Y,\sigma} := \mathcal{N}(0,EE^T+\sigma^2 I_d).
$
Given this distribution, we assume that we have perfectly learned the score:
$
s_\sigma(x) := \nabla \log p_{Y,\sigma}(x) = -\bigl(EE^T+\sigma^2I_d\bigr)^{-1}x.
$
Our goal is to distill this distribution into a distribution 
$
p_{G_\theta} := (G_\theta)_\sharp \mathcal{N}(0,I_d)
$
given by the push-forward of \(\mathcal{N}(0,I_d)\) by a generative network \(G_\theta : \mathbb{R}^d \to \mathbb{R}^d\). To model a U-Net \cite{ronneberger2015u} style architecture with a low-rank structure, we consider maps \(G_\theta\) with \(\theta = (U,V)\) of the form
$
G_\theta(z) := U V^T z,
$
where
$
U \in \mathbb{R}^{d \times r} ~ \text{with} ~ U^TU=I_r ~ \text{and}~   V \in \mathbb{R}^{d \times r}.
$
Let
$
\Theta := \{(U,V): U \in \mathrm{St}(d,r),\, V \in \mathbb{R}^{d\times r}\}.
$ Here, \( \mathrm{St}(d, r) \), known as the Stiefel manifold, is the set of all \( d \times r \) matrices with orthonormal columns. 
We then distill the noisy distribution by minimizing the score-based loss (or Fisher divergence) as in \cite{zhou2024score}:
\begin{equation}\label{eq:ideal-score-loss-r}
\min_{\theta\in \Theta} \mathcal{L}(\theta) := \mathbb{E}_{x\sim p_{G_\theta}}\left[\|s_\sigma(x)-\nabla\log p_{G_\theta}(x)\|_2^2\right].
\end{equation}




\subsection{Warm-up case: $r=1$}
We first consider the case where the latent rank  
$r=1$ as a preliminary step and provide a brief outline of the proof.
  Then the data distribution $p_X$ is a  degenerate Gaussian of the form $p_X := \cN(0,e_1e_1^T),$ where $e_1 \in \RR^d$ is the first standard basis vector in $\RR^d$ (any arbitrary unit vector would suffice). 
In this case, we will consider maps $G_{\theta}$ with $\theta = (u,v)$ of the form $G_{\theta}(z) := uv^Tz\ \text{where}\ \theta=(u,v):  \|u\|_2 = 1, v \in \RR^d. $
Let $\mathbb{S}^{d-1} := \{u \in \RR^d : \|u\|_2 = 1\}$ denote the unit sphere in $\RR^d$. Consider the constraint set of parameters $\Theta := \{\theta = (u,v) : (u,v) \in \mathbb{S}^{d-1}\times \RR^d\}.$ The following Theorem \ref{thm:r=1} shows that minimizers of \eqref{eq:ideal-score-loss-r} induce low-rank distributions that have lower Wasserstein-2 distance to the true distribution than the noisy distribution. We also precisely quantify how far these distributions are:
\begin{theorem}[$r=1$]\label{thm:r=1}
    Fix $\sigma > 0$. Consider the distributions $p_X := \cN(0,e_1e_1^T)$ and $p_{Y,\sigma} := \cN(0,e_1e_2^T + \sigma^2I_d)$.\ys{We should not call them `global minimizers`, they are just a set of good optimizers} Then the global minimizer of \eqref{eq:ideal-score-loss-r} over the constraint set $\theta_* \in \Theta$ is precisely   \begin{align*}
        (u_*,v_*) : u_*=e_1\ \quad\text{and} \quad \|v_*\|_2 = \sqrt{1+\sigma^2}\  \label{eq:case1-r=1},
    \end{align*} which induces the distilled distribution
$p_{G_{\theta^*}} = \mathcal{N}(0,(1+\sigma^2)e_1e_1^T).$ For any $d \in \mathbb{N}$, $$W_2^2(p_{G_{\theta_*}},p_X)
         = W_2^2(p_{Y,\sigma},p_X) - (d-1)\sigma^2 <  W_2^2(p_{Y,\sigma},p_X).$$ 
\end{theorem}
A brief proof is presented as follows (see Appendix for more details):
\begin{proof}
  Note that the distance between the noisy distribution $p_{Y,\sigma}$ and the data distribution $p_X$ is given by \begin{align*}
        W_2^2(p_{Y,\sigma},p_X) = 2+\sigma^2 -2\sqrt{1+\sigma^2} + (d-1)\sigma^2.
    \end{align*} 
    % We then try to find the global minimizes of \eqref{eq:ideal-score-loss-r} and calculate $W_2^2(p_{G_{\theta_*}},p_X)$.
    
     Observe that for $\theta = (u,v)$, the induced distribution is $p_{G_{\theta}} = \cN(0,\|v\|_2^2 uu^T).$ Note that the score function of $p_{G_{\theta}}$ is well-defined on $\mathrm{span}(u)$ and is given by $
        \nabla \log p_{G_{\theta}}(x)= -\|v\|_2^{-2}uu^Tx.$ We now simplify the loss function (\ref{eq:ideal-score-loss-r}):  for $\theta$ such that $\|u\|_2 = 1$, we have
    \begin{align*}
       & \cL(\theta)  = \EE_{x \sim p_G}\left[\|s_{\sigma}(x) - \nabla \log p_{G_{\theta}}(x)\|_2^2\right] \\
        & = \EE_{x \sim p_G}\left[\|(e_1e_1^T + \sigma^2 I_d)^{-1}x - \|v\|_2^{-2}uu^Tx\|_2^2\right] \\
        & = \EE_{z \sim \cN(0,I_d)}\left[\|(e_1e_1^T + \sigma^2 I_d)^{-1}uv^Tz - \|v\|_2^{-2}uu^Tuv^Tz\|_2^2\right] \\
        & = \EE_{z \sim \cN(0,I_d)}\left[v^Tz\right]\cdot\|(e_1e_1^T + \sigma^2 I_d)^{-1}u - \|v\|_2^{-2}u\|_2^2 \\
        & = \|v\|_2^2\cdot\|(e_1e_1^T + \sigma^2 I_d)^{-1}u - \|v\|_2^{-2}u\|_2^2,
    \end{align*} where we used $\|u\|_2 = 1$ in the fourth equality and the fact that $v^Tz \sim \cN(0,\|v\|_2^2)$ for $z \sim \cN(0,I_d)$ in the final equality. Thus, in order to minimize this loss we must have that \begin{align*}
        (e_1e_1^T + \sigma^2 I_d)^{-1}u = \|v\|_2^{-2}u.
    \end{align*} That is, $(u,\|v\|_2^{-2})$ must be an eigenpair of the matrix $(e_1e_1^T + \sigma^2 I_d)^{-1}.$ 
One can easily show that the global minimizer is given by the top eigenpair (see Appendix for more details), i.e., $$u_*=e_1,\|v_*\|_2=\sqrt{1+\sigma^2}.$$ 
 As a result,  $p_{G_{\theta_*}} = \cN(0,(1+\sigma^2)e_1e_1^T).$ 
 In addition, the Wasserstein-2 distance between the distilled distribution $p_{G_{\theta^*}}$ and the data distribution $p_X$ is  \begin{align*}
        W_2^2(p_{G_{\theta_*}},p_X) & = 2+\sigma^2 - 2\sqrt{1+\sigma^2} \\
        & = W_2^2(p_{Y,\sigma},p_X) - (d-1)\sigma^2 \\
        & < W_2^2(p_{Y,\sigma},p_X).
    \end{align*}
\end{proof}
\begin{remark}
    The optimal solution requires $U^*$ to capture the direction of $e_1$, which is also the top eigenvector of the covariance matrix of the clean data distribution. 
    \end{remark}
    \begin{remark}
Distillation acts as an implicit regularization for the learned noisy distribution by enforcing the one-step generator to focus on the direction of the principal eigenvector.
    \end{remark}


\subsection{Extension to general 
$r$}
We provide the theorem \ref{thm:general-r} for general $r$ as follows (see Appendix for proof):
\begin{theorem}[General rank \(r\)]\label{thm:general-r}
Fix \(\sigma>0\). Consider the distributions $p_X := \cN(0,EE^T)$ and $p_{Y,\sigma} := \cN(0,EE^T + \sigma^2I_d)$. 
\ys{We should not call them `global minimizers`, they are just a set of good optimizers} Then the global minimizer  of \eqref{eq:ideal-score-loss-r} over \(\Theta\)  is given by
$$\label{eq:good-case}
U = E \quad (\text{up to an orthogonal transformation}) \quad \text{and} \quad V^TV = (1+\sigma^2)I_r,
$$
which induces the distilled distribution
$p_{G_{\theta^*}} = \mathcal{N}(0,(1+\sigma^2)EE^T).$ 
Moreover, one can verify that for any $d \in \mathbb{N}$, 
\[
W_2^2(p_{G_{\theta^*}},p_X) = W_2^2(p_{Y,\sigma},p_X) - (d-r)\sigma^2 <  W_2^2(p_{Y,\sigma},p_X).
\]
\end{theorem}
\begin{remark}
    The Wasserstein-2 distance gap decreases from $(d-1)\sigma^2$ to $(d-r)\sigma^2$ in the general rank $r$ case. Note that  the assumption of a low-rank structure of image data, i.e. $r <d$, is widely accepted. 
\end{remark}
\begin{remark}
    The optimal solution requires $U^*$ to capture all  the orthogonal bases in $E$, which are the top eigenvectors of the covariance matrix of the clean data distribution with non-zero eigenvalues. 
    \end{remark}
    \begin{remark}
Distillation acts as an implicit regularization for the learned noisy distribution by enforcing the one-step generator to focus on the direction of the principal eigenvectors with non-zero eigenvalues.
    \end{remark}

\subsection{Toy example}

A toy example is provided to demonstrate the implicit regularization effects brought by distillation on the learned data distribution in Fig \ref{fig:toy}.   
The core problem with pretrained diffusion models on the noisy dataset, e.g. (b)Ambient-Full and (c)Ambient Truncated, is that they force the approximating distribution to spread out its probability mass to cover all regions where the target distribution has mass, often at the cost of fidelity in capturing the true shape and separation of the modes.  In contrast, 
(d)DSD excels at denoising the original dataset, producing a narrow, concentrated, and sharp approximation that aligns with our main idea of implicit regularization in Theorem \ref{thm:general-r}.



\begin{figure}[ht]
    \centering
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{toy/noisy_dataset.png}
        \caption{Noisy dataset $\sigma=0.05$}
        \label{fig:sub1}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{toy/full_sampling_sigma_0.05_train_sigma_0.05.png}
        \caption{Ambient-Full}
        \label{fig:sub2}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{toy/truncate_sampling_sigma_0.05_train_sigma_0.05.png}
        \caption{Ambient-Truncated}
        \label{fig:sub3}
    \end{subfigure}
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[width=\linewidth]{toy/4_epoch_292000_sigma_0.05_train_sigma_0.05.png}
        \caption{DSD (one-step)}
        \label{fig:sub4}
    \end{subfigure}
    \caption{\textbf{A toy example of learning from a noisy dataset with $\sigma=0.05$.}   Pretrained diffusion models such as Ambient-Full and  Ambient Truncated tend to force the approximating distribution to spread out its probability mass to cover all regions. DSD excels at denoising the original dataset, demonstrating the implicit regularization effects brought by distillation.  }
    \label{fig:toy}
\end{figure}


% \begin{figure}[htbp]
%     \centering
%     \begin{tabular}{c ccc}
%         & \textbf{Full Sampling} & \textbf{Truncated Sampling} & \textbf{SiD} \\
        
%     \raisebox{2ex}{\rotatebox{90}{\textbf{Train $\sigma=0.0$}}} &
%         \begin{subfigure}{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{toy/full_sampling_sigma_0.05_train_sigma_0.0.png}
%             %\caption{}
%         \end{subfigure} &
%         \begin{subfigure}{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{toy/truncate_sampling_sigma_0.05_train_sigma_0.0.png}
%             %\caption{}
%         \end{subfigure} &
%         \begin{subfigure}{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{toy/1_epoch_221000_sigma_0.05_train_sigma_0.0.png}
%             %\caption{}
%         \end{subfigure} \\
        
%         \raisebox{2ex}{\rotatebox{90}{\textbf{Train $\sigma=0.05$}}} &
%         \begin{subfigure}{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{toy/full_sampling_sigma_0.05_train_sigma_0.05.png}
%             %\caption{}
%         \end{subfigure} &
%         \begin{subfigure}{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{toy/truncate_sampling_sigma_0.05_train_sigma_0.05.png}
%             %\caption{}
%         \end{subfigure} &
%         \begin{subfigure}{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{toy/4_epoch_292000_sigma_0.05_train_sigma_0.05.png}
%             %\caption{}
%         \end{subfigure} \\
        
%         \raisebox{2ex}{\rotatebox{90}{\textbf{Train $\sigma=0.1$}}} &
%         \begin{subfigure}{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{toy/full_sampling_sigma_0.05_train_sigma_0.1.png}
%             %\caption{}
%         \end{subfigure} &
%         \begin{subfigure}{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{toy/truncate_sampling_sigma_0.05_train_sigma_0.1.png}
%             %\caption{}
%         \end{subfigure} &
%         \begin{subfigure}{0.3\textwidth}
%             \centering
%             \includegraphics[width=\linewidth]{toy/22_epoch_299000_sigma_0.05_train_sigma_0.1.png}
%             %\caption{}
%         \end{subfigure} \\
%     \end{tabular}
%     \label{fig:3x3grid}
%     \caption{The generation method is evaluated using different training $\sigma$levels, while the training dataset is fixed at $\sigma=0.05$. The plot illustrates the impact of underestimating or overestimating the $\sigma$ level on various generation methods.}
% \end{figure}

